Instability of Self-Driving Satellite Mega-Constellation: From Theory to Practical Impacts on Network Lifetime and Capacity

Low Earth Orbit (LEO) satellite mega-constellations aim to enable high-speed Internet for numerous users anywhere on Earth. To safeguard their network infrastructure in congested outer space, they perform automatic orbital maneuvers to avoid collisions with external debris and satellites. However, our control-theoretic analysis and empirical validation using Starlink's space situational awareness datasets discover that, these safety-oriented maneuvers themselves can threaten safety and networking via cascaded collision avoidance inside the mega-constellation. This domino effect forces a dilemma between long-term LEO network lifetime and short-term LEO network capacity. Its root cause is that, the decades-old local pairwise maneuver paradigm for standalone satellites is inherently unstable if scaled out to recent mega-constellation networks. We thus propose an alternative bilateral maneuver control that stabilizes self-driving mega-constellations for concurrent network lifetime and capacity boosts. Our operational trace-driven emulation shows a 8$\times$ network lifetime extension in Starlink without limiting its network capacity.

==> theory-definition.tex <==
\subsection{Definition of Stability}
\label{subsec:define}
\p{In this section, we give the mathematical definition of stability and a constellation-specific definition, including equilibrium points. We should emphasize the physical meaning and significance of stability for constellations. }

==> theory-method.tex <==
\subsection{Stability Assessment Method}
\label{subsec:method}
\p{In this section, we introduce our method to assess the stability and give a concise formula expression. It is necessary to clarify the physical meaning of each parameter, that is, what behavior it corresponds to in an autonomous driving system.}
